Persona2vec: A Flexible Multi-role Representations Learning Framework for Graphs

Graph embedding techniques, which learn low-dimensional representations of a graph, are achieving state-of-the-art performance in many graph mining tasks. Most existing embedding algorithms assign a single vector to each node, implicitly assuming that a single representation is enough to capture all characteristics of the node. However, across many domains, it is common to observe pervasively overlapping community structure, where most nodes belong to multiple communities, playing different roles depending on the contexts. Here, we propose persona2vec, a graph embedding framework that efficiently learns multiple representations of nodes based on their structural contexts. Using link prediction-based evaluation, we show that our framework is significantly faster than the existing state-of-the-art model while achieving better performance.

==> algorithm.tex <==
\subsection{Algorithm}

Here we describe our algorithm.

\begin{algorithm}[t!]
	\caption{Refined ego-splitting. Our method for generating the persona graph} 
	\label{alg:ego_splitting} 
	\begin{algorithmic}[1]
		\Require{}
		\Statex{$G(V,E)$, the graph}
		\Statex{$\lambda$, weight of persona edges}
		\Statex{$\mathcal{C}$}, non-overlapping local clustering algorithm
		\Ensure{}
		\Statex{$G_P(V_P, E_P)$, the persona graph}
		\algrule
		\Function{RefEgoSplit}{$G$}
		\For{{\textbf{each} $v_o \in V$}}
		    \State $P_{v_o} \leftarrow \mathcal{C}(v_o)$ \Comment{find local clusters of $v_o$}
		    \For{{\textbf{each} $p \in P_{v_o}$}}
		        \State Create $v_p$ \Comment{create persona nodes for local clusters}
		    \EndFor
		    \For{{\textbf{each} $p \in P_{v_o}$}}
    		    \For{{\textbf{each} $d \in P_{v_o}$}}
    		        \State Add persona edge between $p$ and $d$
    		        \State Set edge weight to $\lambda$
    		    \EndFor
		    \EndFor
		\EndFor			
		
		\For{{\textbf{each} $v_p$ in $V_P$}}
    		\For{{\textbf{each} $v_d \in V_P$}}
    		    \If{$(v_p, v_d) \in E$ and $v_p, v_d$ belong to same $P_{v_o}$}
    		        \State Add real edge between $v_p$ and $v_d$
    		        \State Set edge weight to $1$
    		    \EndIf
    		\EndFor
		\EndFor
		\State{\Return $G_P(V_P, E_P)$}
		\EndFunction
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t!]
	\caption{\pv{}. Our method for generating node representations under different different contexts.}
	\label{alg:persona2vec} 
	\begin{algorithmic}[1]
		\Require{}
		\Statex{$G(V,E)$, the graph}
		\Statex{$d$, embedding dimension}
		\Statex{$\mathcal{\gamma}_b$, number of walks per node for base embedding}
		\Statex{$t_b$, random walk length for base embedding}
		\Statex{$w_b$, window size for base embedding}
		\Statex{$\mathcal{\gamma}_p$, number of walks per node for persona embedding}
		\Statex{$t_p$, random walk length for persona embedding}
		\Statex{$w_p$, window size for persona embedding}
		\Statex{$\alpha$, learning rate}		
		\Statex{\textsc{EmbeddingFunc}, a graph embedding method e.g. DeepWalk, node2vec}
		\Ensure{}
		\Statex{$\Phi_{G_P}$, a matrix with one representation for each persona node}
		\algrule
		\Function{\pv{}}{$G$, $\textsc{EmbeddingFunc}$}
		\State{$G_{P} \leftarrow \textsc{RefEgoSplit}(G)$}
		\Comment{Create the refined persona graph $G_P$ of $G$. }
		
	
		% Learn persona embeddings		
		\For{$i=0$ to $\mathcal{\gamma}$}
			\State	$\mathcal{O} = \text{Shuffle}(V_{G_P})$
	        \For{\textbf{each} $v_i \in \mathcal{O}$}
				\State $\mathcal{W}_{v_i} = WeightedRandomWalk(G_P, v_i, $t$) $		
			\EndFor						
		\EndFor			
		
		\State{$\Phi_{G_P} \leftarrow \textsc{EmbeddingFunc}(\alpha, \mathcal{W}, w, d, \gamma, t)$}
		\Comment{Embed persona graph}	
		
		\State{\Return $\Phi_{G_P}$}
		\EndFunction
	\end{algorithmic}
\end{algorithm}
